Implicit Dimension Identification in User-Generated Text with LSTM Networks

In the process of online storytelling, individual users create and consume highly diverse content that contains a great deal of implicit beliefs and not plainly expressed narrative. It is hard to manually detect these implicit beliefs, intentions and moral foundations of the writers. We study and investigate two different tasks, each of which reflect the difficulty of detecting an implicit user's knowledge, intent or belief that may be based on writer's moral foundation: 1) political perspective detection in news articles 2) identification of informational vs. conversational questions in community question answering (CQA) archives and. In both tasks we first describe new interesting annotated datasets and make the datasets publicly available. Second, we compare various classification algorithms, and show the differences in their performance on both tasks. Third, in political perspective detection task we utilize a narrative representation language of local press to identify perspective differences between presumably neutral American and British press.

==> 3_Method.tex <==
\section{Method}
\label{sec:method}

%%% where is teh intuition of why LSTM is suitable for this problem

In the course of this research we focus on the identification of implicit dimensions in user-generated text.
We treat this as a classification problem and train an LSTM network classifier, which classifies the given piece of text as an appropriate dimension's class. In the case of CQA task, the question is classified in either \textit{informational} or \textit{conversational} class. In NEWS task, the article is classified as either the \textit{Israeli-Perspective} or \textit{Palestinian Perspective} class.

During our experiments we start with several baseline algorithms, and then in order to improve performance, we use an LSTM network. 

\subsection{Architecture}

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.7\textwidth]{LSTMgeneral.png}
    \caption{The LSTM network architecture for a binary classification task.} 
    \label{fig:general}
\end{figure}
\FloatBarrier


Figure \ref{fig:general} presents the general architecture of an LSTM network for the classification task. In each step $i$, the corresponding input vector $x_i$ representing a word in the piece of text is fed into the network.  At the final step $n$, the LSTM's state is \textit{squashed} with the sigmoid function in a value ranging from zero to one. Because both of our classification problems, are binary classification problems we give the network's output a probabilistic interpretation, of belonging to one of the two classes.  Finally the result is used to compute the cross entropy loss function.


\begin{figure}[h!]
    \centering
    \includegraphics[width=0.9\textwidth]{LSTMbias.png}
    \caption{The political perspective detection model architecture with an example title. } 
    \label{fig:bias}
\end{figure}
\FloatBarrier
Figure \ref{fig:bias} presents the architecture of the LSTM network, which we use to identify the implicit dimension in a political perspective. In this example, a political perspective within international newswire. The title is taken from an article\footnote{\url{https://www.timesofisrael.com/hezbollah-mp-urges-kidnapping-israeli-civilians-in-next-war/}} which appeared in the Times of Israel. In each step, a word from an article's title was fed into the network, embedding was learned, and the classification was made after the last word for a given title. In this case, only the value from the last step is considered into the loss function computation, in contrast to standard RNN, as was previously explained in the Background section of this paper.


\begin{figure}[h!]
    \centering
    \includegraphics[width=0.9\textwidth]{LSTM_zoom_bias.png}
    \caption{The perspective detection model architecture explained: a zoom in.} 
    \label{fig:bias_zoom}
\end{figure}
\FloatBarrier


Figure \ref{fig:bias_zoom} presents the LSTM-network architecture, in greater detail, during the training process. In each time stamp $t$ the following process occurs:
\begin{itemize}
\item A word which is represented as a one-hot vector is fed into the network.
\item A dense word representation, the word's embedding in a dense vector space is learned.
\item The word's embedding is fed into the LSTM memory cell, and all of the LSTM's equations are computed based on it's previous hidden state and memory cell value.
\end{itemize}

In the last word of a piece of text, the LSTM output is transformed into a single value scalar with MLP, thereby squashing its output value to a range from zero to one with a \textit{logistic sigmoid} function. This output is given a probabilistic interpretation and is used to compute the cross-entropy loss function.

The classification process is performed in an analogous way, without computing the loss. The last word of a piece of text is fed into the network, and the MLP's output value is used for the classification. If the value is above 0.5 then the class 1 is set as the current text's class. Otherwise, the second class is assumed.


%\subsection{Training paradigms}

%Labeled dataset. k-fold cross validation.
%Using portions of unlabeled data.

%\subsection{Batch train}

%In this subsection we describe the batch training paradigms.

%\subsection{Bidirectional LSTM for classification}

%Bidirectional LSTM shown an improvement in several tasks - such as sequence-to-sequence, and POS-tagging. In our case, there was not any improvement in both task we study in the course of this research.

%\begin{figure}[h!]
%    \centering
%    \includegraphics[width=0.7\textwidth]{bilstm_classification.png}
%   \caption{The architecture of a bidirectional LSTM for classification. The final states of each LSTM are concatenated into a single representation, that can be seen as a complete text-piece embedding. Finally this embedding is classified with an MLP which was trained specifically for this task.} 
%    \label{fig:bilstm}
%\end{figure}
%\FloatBarrier
